Nonlinear Inductive Matrix Completion based on One-layer Neural Networks

The goal of a recommendation system is to predict the interest of a user in a given item by exploiting the existing set of ratings as well as certain user/item features. A standard approach to modeling this problem is Inductive Matrix Completion where the predicted rating is modeled as an inner product of the user and the item features projected onto a latent space. In order to learn the parameters effectively from a small number of observed ratings, the latent space is constrained to be low-dimensional which implies that the parameter matrix is constrained to be low-rank. However, such bilinear modeling of the ratings can be limiting in practice and non-linear prediction functions can lead to significant improvements. A natural approach to introducing non-linearity in the prediction function is to apply a non-linear activation function on top of the projected user/item features. Imposition of non-linearities further complicates an already challenging problem that has two sources of non-convexity: a) low-rank structure of the parameter matrix, and b) non-linear activation function. We show that one can still solve the non-linear Inductive Matrix Completion problem using gradient descent type methods as long as the solution is initialized well. That is, close to the optima, the optimization function is strongly convex and hence admits standard optimization techniques, at least for certain activation functions, such as Sigmoid and tanh. We also highlight the importance of the activation function and show how ReLU can behave significantly differently than say a sigmoid function. Finally, we apply our proposed technique to recommendation systems and semi-supervised clustering, and show that our method can lead to much better performance than standard linear Inductive Matrix Completion methods.

==> app.tex <==
\begin{comment}
\section{Applications}\label{sec:app}
\subsection{Semi-supervised Clustering}
In the semi-supervised clustering problem, we are given a set of items with their features, $X\in \dR^{n\times d}$, where $n$ is the number of items and $d$ is the feature dimension, and an incomplete similarity matrix $A$, where $A_{i,j} = 1$ if $i$-th item and $j$-th item are similar and $A_{i,j} = 0$ if $i$-th item and $j$-th item are dissimilar. The goal is to do clustering based on the features and the partially observed similarity matrix. This problem has been formulated as an IMC problem \cite{yi2013semi}, which is shown to outperform other approaches. We can also easily apply our model Eq.~\eqref{eq:base_model} to this problem. We'll show experimental results on this application in Sec.~\ref{sec:exp}. 
%More specifically, as in the general framework, Eq.~\eqref{eq:general_nimc}, we will $x=y$, we can also set $\mathcal{U}=\mathcal{V}$w. \cite{ noisy_imc, gimc} used this application for the case when the features are noisy \cite{ noisy_imc} or the boundary is nonlinear \cite{gimc}. 
If we constrain the latent space $\mathcal{S}$ to be non-negative by taking $\phi$ to be ReLU or sigmoid and let $k$ be the number of clusters, then the results will have interpretability: the normalized $\phi(U^\top x)$ can be viewed as the probability of $x$ to be assigned to each cluster. 

\subsection{Low-rank Multi-label and Multi-class Learning via Nonlinear Mapping}
Multi-label and Multi-class problems with a large number of labels/classes can be formulated as an IMC problem, e.g. \cite{yu2014large}. Let $A_{i,j} = 1$ if sample $i$ belongs to label $j$.  We can assume $A_{i,j} \approx \mathcal{U}(x_i)^\top v_j $, where $x_i$ is the feature vector and $v_j$ is the latent feature vector of label $j$.  %In the general framework, Eq.~\eqref{eq:general_nimc}, $v_j = Ve_j$, where $\mathcal{V}$ is represented by a matrix $V$. 
\cite{yu2014large} used linear mapping for $\mathcal{U}$ and \cite{si2016goal} used a three-layer neural network for $\mathcal{U}$. \cite{yu2014large} derived generalization bound, while \cite{si2016goal} achieves  better experimental results but without theoretical guarantees. 

\subsection{Non-negative Matrix Factorization with Side Information}
Non-negative Matrix Factorization (NMF) has numerous applications. When side information is available, we can also leverage them and obtain a better factorization \cite{mei2017nonnegative}. In our framework, a non-negative link function can be added before the output of $\mathcal{U}$ to ensure the non-negativity. ReLU and sigmoid naturally fit in this task.  

\subsection{Recommender System using Deep Neural Networks}
For highly structured data, such as images and speech, we typically require neural networks to process them. To use framework Eq.~\eqref{eq:general_nimc}, replace $\mathcal{U},\mathcal{V}$ by neural networks. These neural-network-based recommender systems have achieved great practical success in large dataset, such as Youtube \cite{covington2016deep}, web search \cite{huang2013learning}. 

\end{comment}

==> preli.tex <==
\section{Notation}

For any positive integer $n$, we use $[n]$ to denote the set $\{1,2,\cdots,n\}$.
For random variable $X$, let $\mathbb{E}[X]$ denote the expectation of $X$ (if this quantity exists).
%Define $W := [ w_1, w_2,\cdots, w_K] \in \R^{K\times d}$ and $ v := [v_1;\cdots;v_K]$. 
%We use $\Expect{X}$ to denote the expectation of a random variable $X$.
For any vector $ x\in \mathbb{R}^n$, we use $\|  x\|$ to denote its $\ell_2$ norm.

We provide several definitions related to matrix $A$.
Let $\det(A)$ denote the determinant of a square matrix $A$. Let $A^\top$ denote the transpose of $A$. Let $A^\dagger$ denote the Moore-Penrose pseudoinverse of $A$. Let $A^{-1}$ denote the inverse of a full rank square matrix. Let $\| A\|_F$ denote the Frobenius norm of matrix $A$. Let $\| A\|$ denote the spectral norm of matrix $A$. Let $\sigma_i(A)$ to denote the $i$-th largest singular value of $A$.

We use $\bone_{f}$ to denote the indicator function, which is $1$ if
$f$ holds and $0$ otherwise. Let $I_d \in \mathbb{R}^{d\times d}$
denote the identity matrix. We use $\phi(z)$ to denote an activation
function. We define $(z)_+:= \max \{ 0,z\}$. We use ${\cal D}$ to
denote a Gaussian distribution ${\cal N}(0,I_d)$ or to denote a joint
distribution of $(X,Y)\in \mathbb{R}^d\times\mathbb{R}$, where the
marginal distribution of $X$ is ${\cal N}(0,I_d)$. For integer $k$, we
use $\D_k$ to denote $\N(0,I_k)$.

For any function $f$, we define $\widetilde{O}(f)$ to be $f\cdot \log^{O(1)}(f)$. In addition to $O(\cdot)$ notation, for two functions $f,g$, we use the shorthand $f\lesssim g$ (resp. $\gtrsim$) to indicate that $f\leq C g$ (resp. $\geq$) for an absolute constant $C$. We use $f\eqsim g$ to mean $cf\leq g\leq Cf$ for constants $c,C$.


\begin{definition}
Let $\alpha_q (\sigma) = \E_{z\sim \N(0,1)} [\phi'(\sigma \cdot z) z^q], \forall q \in \{0,1,2\}$, and $\beta_q (\sigma)= \E_{z\sim \N(0,1)} [\phi'^2(\sigma \cdot z) z^q], \forall q\in \{0,2\}$. Let $\gamma_q (\sigma) = \E_{z\sim \N(0,1)} [ \phi(\sigma \cdot z) z^q]$, $\forall q\in \{0,1,2,3,4\}$.
\end{definition}

\section{Preliminaries}

